Graph Sparsification for Derandomizing Massively Parallel Computation with Low Space

The Massively Parallel Computation (MPC) model is an emerging model which distills core aspects of distributed and parallel computation. It has been developed as a tool to solve (typically graph) problems in systems where the input is distributed over many machines with limited space. Recent work has focused on the regime in which machines have sublinear (in $n$, the number of nodes in the input graph) memory, with randomized algorithms presented for fundamental graph problems of Maximal Matching and Maximal Independent Set. However, there have been no prior corresponding \emph{deterministic} algorithms. A major challenge underlying the sublinear space setting is that the local space of each machine might be too small to store all the edges incident to a single node. This poses a considerable obstacle compared to the classical models in which each node is assumed to know and have easy access to its incident edges. To overcome this barrier we introduce a new \emph{graph sparsification technique} that \emph{deterministically} computes a low-degree subgraph with additional desired properties. Using this framework to derandomize the well-known randomized algorithm of Luby [SICOMP'86], we obtain $O(\log \Delta+\log\log n)$-round \emph{deterministic} MPC algorithms for solving the fundamental problems of \emph{Maximal Matching} and \emph{Maximal Independent Set} with $O(n^{\epsilon})$ space on each machine for any constant $\epsilon > 0$. Based on the recent work of Ghaffari et al. [FOCS'18], this additive $O(\log\log n)$ factor is \emph{conditionally} essential. These algorithms can also be shown to run in $O(\log \Delta)$ rounds in the closely related model of \congc, improving upon the state-of-the-art bound of $O(\log^2 \Delta)$ rounds by Censor-Hillel et al. [DISC'17].

==> improved-mis.tex <==
%---------------------------------------------------------------------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Improved derandomization in the congested clique model}

\begin{lemma}
For $\Delta \le 2^{\sqrt{\log n}}$ can compute MIS in $O(\log\log\Delta)$ deterministic congested clique rounds.
\end{lemma}
\begin{proof}
The algorithm first collects the $O(\log \Delta)$-ball of each vertex. Then, each of the $O(\log \Delta)$ randomized rounds require seed of size $\log \Delta$. Since $\log^2 \Delta \le \log n$, we can compute the desired seed in $O(1)$ rounds. After de-randomizing the $O(\log \Delta)$ phases, we are left with subgraph of size $O(n)$, which can be solved on a single machine.
\end{proof}


\begin{lemma}
Given a degree parameter $\Delta$, one can have a recursive degree reduction procedure that partitions the graph into vertex-disjoint subgraphs of degree at most $\Delta$ (and their corresponding palettes) in $O(\log n/\log \Delta)$ rounds.
\end{lemma}
We next sketch a $(1+\epsilon)\Delta$ list coloring algorithm that works in $(\log n)^{1/3}$ rounds. 
Let $\Delta=2^{(\log n)^{2/3}}$. Then by the above lemma, we can partition the graph into independent coloring instances with maximum degree $\Delta$ in $O((\log n)^{1/3})$. 


We will use the $O(\log \Delta)$ algorithm (say of Ghaffari) by compressing $\sqrt{\log \Delta}=(\log n)^{1/3}$
using $O(\log\log n)$ rounds. For each round, we need to find a seed of $O(\log \Delta)$ bits.
This gives a total of $\log \Delta \cdot \sqrt{\log \Delta}=O(\log n)$ bits which can be derandomized in $O(1)$. 

Since the shattering effect of Ghaffari's algorithm works in the congested clique, for the MPC with sub-linear space setting, we will have a different approach. We will derandomize the $O(\sqrt{\log n})$ round algorithm for $(1+\epsilon)\Delta$ coloring, that works as follows. For $O(\sqrt{\log n})$ rounds, each vertex picks a color uniformly at random. One can show that after $\sqrt{\log n}$ rounds, w.h.p. there is no path of length $O(\sqrt{\log n})$ that is entirely uncolored. This implies that the radius of each uncolored component is $\sqrt{\log n}$. 
Once the degree is reduced to $2^{\sqrt{\log n}}$ using the above lemma in $O(\sqrt{\log n})$ rounds,  we can indeed collect the ball of radius $O(\sqrt{\log n})$. Note that each step of the randomized procedure requires just $\sqrt{\log n}$-wise independent. Overall, we will need to compute $O(\sqrt{\log n}\log n)$ bits which can be done in $O(\sqrt{\log n})$ rounds. (To do that derandomization procedure, we will aim at minimizing the number of paths of length $\ell=\sqrt{\log n}$ that are fully uncolored. Each vertex $v$ will take into account all the paths of length $\ell$ that start at $v$.)

%---------------------------------------------------------------------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------------------------------------------------------------------





